GaussNav: Gaussian Splatting for Visual Navigation

In embodied vision, Instance ImageGoal Navigation (IIN) requires an agent to locate a specific object depicted in a goal image within an unexplored environment. The primary challenge of IIN arises from the need to recognize the target object across varying viewpoints while ignoring potential distractors. Existing map-based navigation methods typically use Bird's Eye View (BEV) maps, which lack detailed texture representation of a scene. Consequently, while BEV maps are effective for semantic-level visual navigation, they are struggling for instance-level tasks. To this end, we propose a new framework for IIN, Gaussian Splatting for Visual Navigation (GaussNav), which constructs a novel map representation based on 3D Gaussian Splatting (3DGS). The GaussNav framework enables the agent to memorize both the geometry and semantic information of the scene, as well as retain the textural features of objects. By matching renderings of similar objects with the target, the agent can accurately identify, ground, and navigate to the specified object. Our GaussNav framework demonstrates a significant performance improvement, with Success weighted by Path Length (SPL) increasing from 0.347 to 0.578 on the challenging Habitat-Matterport 3D (HM3D) dataset. The source code is publicly available at the link: https://github.com/XiaohanLei/GaussNav.

==> tables/gauss_construct_results.tex <==
\begin{table}[tb]
  \centering
  \caption{}
  \label{tab:gauss_construct_result}
  \resizebox{\linewidth}{!}{
  \begin{tabular}{@{}cccccccccccccccccccccccccccccccc@{}}
    \toprule
    Scene Index & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 & 30 \\
    \midrule
    Avg. PSNR & 19.36 & 7.59 & 19.50 & 13.98 & 34.71 & 7.53 & 21.39 & 14.20 & 26.25 & 28.42 & 4.96 & 32.97 & 37.08 & 10.24 & 20.48 & 29.25 & 18.57 & 27.69 & 10.01 & 6.95 & 12.48 & 28.22 & 12.34 & 36.83 & 14.24 & 32.16 & 11.27 & 10.14 & 10.56 & 41.02 & 35.86 \\
    Avg. Depth L1 & 0.03 & 1.28 & 0.06 & 0.51 & 0.00 & 1.72 & 0.05 & 0.11 & 0.02 & 0.01 & 1.18 & 0.00 & 0.00 & 1.45 & 0.12 & 0.00 & 0.10 & 0.01 & 0.13 & 2.44 & 0.40 & 0.00 & 0.44 & 0.00 & 0.14 & 0.01 & 1.12 & 1.08 & 0.75 & 0.00 & 0.01 \\
    Avg. MS-SSIM & 0.79 & 0.28 & 0.78 & 0.64 & 0.95 & 0.32 & 0.83 & 0.28 & 0.96 & 0.97 & 0.00 & 0.98 & 0.99 & 0.33 & 0.83 & 0.94 & 0.67 & 0.92 & 0.28 & 0.23 & 0.36 & 0.95 & 0.50 & 0.99 & 0.48 & 0.98 & 0.12 & 0.10 & 0.36 & 1.00 & 0.99 \\
    Avg. LPIPS & 0.20 & 0.71 & 0.26 & 0.65 & 0.23 & 0.78 & 0.25 & 0.77 & 0.04 & 0.06 & 0.90 & 0.03 & 0.26 & 0.69 & 0.20 & 0.10 & 0.71 & 0.14 & 0.91 & 0.86 & 0.60 & 0.10 & 0.54 & 0.04 & 0.63 & 0.05 & 0.76 & 0.96 & 0.80 & 0.02 & 0.03 \\
    \bottomrule
  \end{tabular}
  }
  % \vspace{-10pt}
\end{table}
  
